PSRFlow: Probabilistic Super Resolution with Flow-Based Models for Scientific Data

Although many deep-learning-based super-resolution approaches have been proposed in recent years, because no ground truth is available in the inference stage, few can quantify the errors and uncertainties of the super-resolved results. For scientific visualization applications, however, conveying uncertainties of the results to scientists is crucial to avoid generating misleading or incorrect information. In this paper, we propose PSRFlow, a novel normalizing flow-based generative model for scientific data super-resolution that incorporates uncertainty quantification into the super-resolution process. PSRFlow learns the conditional distribution of the high-resolution data based on the low-resolution counterpart. By sampling from a Gaussian latent space that captures the missing information in the high-resolution data, one can generate different plausible super-resolution outputs. The efficient sampling in the Gaussian latent space allows our model to perform uncertainty quantification for the super-resolved results. During model training, we augment the training data with samples across various scales to make the model adaptable to data of different scales, achieving flexible super-resolution for a given input. Our results demonstrate superior performance and robust uncertainty quantification compared with existing methods such as interpolation and GAN-based super-resolution networks.

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> tex/1_introduction_old.tex <==
\section{Introduction}
% [the need for high-quality particle data] visualize particles at high resolution. 
Particle simulations are used to model a wide range of phenomena in fields such as chemistry, physics, and astronomy to help scientists get insights into complex physical systems.
% the behavior of gases, the movement of fluids, the dynamics of chemical reactions, the behavior of biological systems, and the motion of celestial objects. 
High-resolution visualization of particle data is crucial for understanding and interpreting the scientific phenomena behind simulations. However, conducting large-scale simulations is often challenging due to the high computation and memory costs. 
In particular, the appropriate simulation parameters are often unknown and as a result, scientists need to run simulations multiple times with different parameter settings. 
One way to reduce the computational cost is to run the simulation at a low resolution spatially or temporally, and upsample the low-resolution output to the desired resolution during visualization and post-hoc analysis. 

% limitations of existing methods for particle super-resolution: 
% 1. interpolation smoothness; 
% 2. DL: GANs, hard to choose a proper (not too strong) discriminator;
% 3. deterministic one-to-one mappings and lack of uncertainty quantification
While many super-resolution methods have been proposed for volumetric data in the scientific visualization field [\cite{}], fewer have been proposed for particle data. The interpolation-based particle super-resolution methods [\cite{}], which rely on smoothness assumptions, are relatively simple and computationally efficient. However, due to the sparse and irregular nature of particles, interpolation-based methods are insufficient to determine the accurate locations and attributes of the newly sampled particles. The super-resolved results tend to be blurred and lack details. For example, sharp features or feature boundaries that were not adequately captured by the low-resolution particles can not be recovered. % since it can only generate information that is already presented in the low-resolution data. 
Although deep learning-based super-resolution methods have shown great performance in modeling the correspondence between low-resolution and high-resolution pairs for volumetric data [\cite{}], several limitations still need to be addressed before deploying them for particle data. 
Firstly, irregular and unordered particle data pose a challenge for modeling the complex mappings between low and high-resolution particle pairs using convolution operations designed for regular data. A convolution operation tailored for irregular particle data is required. 
Secondly, although generative adversarial networks (GANs) are widely employed for volumetric super-resolution tasks, researchers have found it hard to find a proper not-too-strong discriminator for particle data [\cite{}] as the discriminator tends to optimize faster than the generator, resulting in mode collapse and generating artifacts [\cite{}]. An alternative generative model is needed for high-quality particle super-resolution. 
Thirdly, current super-resolution methods for scientific data are deterministic one-to-one mappings between low and high-resolution data pairs without considering the uncertainties of the super-resolved data. Particle super-resolution is a challenging ill-posed problem due to the inherent difficulties in recovering missing information. As a result, multiple high-resolution outputs may correspond to the same low-resolution input. Thus, it is necessary to perform uncertainty quantification to provide scientists with reliable indications of the super-resolution quality for scientific visualization applications. 
% modeling the missing information 

% spatial distribution does not follow any simple pattern
% [proposed approach of using probabilistic normalizing flow models for particle super-resolution and explain the contribution of this work in addressing the limitations of existing methods.] 
% model uncertainty and generate diverse outputs.
In this paper, we propose {\sysname}, a novel probabilistic approach for particle super-resolution based on the invertible normalizing flows (NFs). By modeling the distribution of high-resolution particles conditioned on low-resolution particles through a multi-scale normalizing flow architecture, we can overcome the limitations of existing techniques. 
First, we treat particle super-resolution as a conditional generation process. A conditional convolutional network for irregular particle data is adopted to fuse low-resolution information into the latent space of high-resolution data. 
Second, different from other generative models, normalizing flows are built on a sequence of invertible mappings between the input data distribution and a simple latent space distribution. They can be trained by directly optimizing the exact likelihood of high-resolution data conditioned on low-resolution data using the change of variables formula. Unlike GANs, normalizing flows are easier to train and are more stable. % unlike autoregressive models, they are also capable of efficient inference. 
Third, instead of the deterministic one-to-one mapping between low and high-resolution particle sets, we incorporate uncertainty quantification into the super-resolution process to make our method more robust and aware of potential errors. 

% [key contributions]: generate high-quality super-res particle data; ability to model uncertainty; adaptability across scales;
Our {\sysname} is an invertible framework that models the conditional relationships between low-resolution particles and high-resolution ones. 
More specifically, in the forward process of {\sysname}, high-resolution particles in the original data distribution are gradually transformed into a conditional latent space with a simpler distribution (e.g., Gaussian) and a latent vector that encodes the low-resolution information. 
During the inverse process, the missing high-frequency information can be sampled from the Gaussian latent space conditioned on the low-resolution particles. 
The conditional generation of high-resolution particles is made by combining the missing high-frequency information with the low-resolution input and leveraging the invertible transformations of {\sysname} to transform the combined information in latent space to the data space.
Given a low-resolution particle set, based on the learned distribution mappings, our model can sample multiple high-resolution particle sets. 
% In contrast to the conventional methods, our method allows exploring the super-resolved particle space. 
% other than the negative log-likelihood loss, we have other losses that add constraints in the latent space of the flow model.
We add a global feature coupling layer to enhance the expressibility of the model for unordered particle data. 
In addition, we augment the training data so that once the model is trained, it can be adaptively applicable for super-resolution across different scales, allowing us to achieve arbitrary power-of-two super-resolution for a given low-resolution input during inference. 

% TALKINGFLOW: TALKING FACIAL LANDMARK GENERATION WITH MULTI-SCALE NORMALIZING FLOW NETWORK. % TALKINGFLOW: good writing
With the trained model, scientists can obtain high-resolution particles and estimate the uncertainties of the super-resolved results. % By transforming data into compact latent representations, similarity comparison or distance computation between data becomes efficient and robust. Also, it reduces the storage cost by only saving the compressed latent representations that can later be used for downstream scientific analysis tasks such as projection, retrieval, feature exploration, clustering, query, etc.
Our qualitative and quantitative evaluation demonstrates that our particle super-resolution method has superior performance compared to bi-linear, cubic, and GAN-based super-resolution methods and provides robust uncertainty quantification.  % of three scientific datasets  % outperforms. superior particle super-resolution performance and robust uncertainty quantification compared to Xs.

In summary, the contributions of our work are threefold:  
\begin{itemize}
\item First, we propose a novel probabilistic particle super-resolution method based on normalizing flow which addresses the limitations of existing techniques. % SR quality
\item Second, our method provides uncertainty quantification to increase the reliability of our super-resolution results.
\item Third, we demonstrate the effectiveness of our approach through experiments on three scientific datasets. 
\end{itemize}

% --------------------------------- End of introduction ----------------------------------------------------------------------------------------- End of introduction  ---------------------------------------------------------------------------------------------------- End of introduction ------------------------------------------------

% For instance, some works utilize latent representations to encode volumes for key time step selection \cite{Porter2019TSselectionTVM}, streamlines clustering \cite{Han2020FlowNet} and isosurfaces comparison \cite{Dai2021IsoExplorerAI}. There are also works utilizing latent space's generation ability to synthesize data for transfer function design \cite{berger2018GanVR} and synthesize fluid simulations \cite{kim2019deepfluids, wiewel2020latentsubdivision, wiewel2019latentphysics}. 

% There are three main challenges when generating a compact but accurate data representation based on scientists' interests. First, it is difficult to represent various types of geometric primitives that scientists may be interested in, such as points, lines, or surfaces, with a unified representation. Second, it is hard to fuse the domain interests into the compact representation. Flexible control of what information should be preserved in the reduced representation is required.
% The existing methods are sophisticatedly designed for a specific type of primitive, such as critical points or isosurfaces. % How to design a unified representation for them still remains an open problem. 


% The first stage is the interest domain controlled latent generation. To generate data representations, we have dual-domain inputs to the Autoencoder, one is the original data and the other is the scientist's interest, represented by a real-valued interest map which has the same size as the data. %  higher value indicating higher interests. 
% To reduce the computational cost for training large-scale volumetric data, we split the original large volume into blocks. Then, each block, together with the corresponding interest domain block, is fed into the Autoencoder. After non-linear transform coding through the encoder, the raw data blocks are converted into latent representations controlled by the interest domain. 
% The second stage is the lossless encoding of latents. After Autoencoder's encoding, we first quantize the generated latents into discrete symbols. Then we apply Asymmetric Numeral Systems (ANS), a kind of entropy encoding algorithm, to losslessly encode the discrete latents into bitstreams for saving. 
% In this process, boring data regions will be encoded with shorter bits compare with while user interested regions will have higher bits. 

% Paragraph 5: pipeline/architecture/framework
% The key to our method is that we explicitly consider user's interest during data reduction. 
% Our workflow of dual-domain latent generation method has two stages, as shown in~\autoref{fig:framework}. 
% The first stage is the interest domain controlled latent generation. To generate data representations, we have dual-domain inputs to the Autoencoder, one is the original data and the other is the scientist's interest, represented by a real-valued interest map which has the same size as the data. %  higher value indicating higher interests. 
% To reduce the computational cost for training large-scale volumetric data, we split the original large volume into blocks. Then, each block, together with the corresponding interest domain block, is fed into the Autoencoder. After non-linear transform coding through the encoder, the raw data blocks are converted into latent representations controlled by the interest domain. 
% The second stage is the lossless encoding of latents. After Autoencoder's encoding, we first quantize the generated latents into discrete symbols. Then we apply Asymmetric Numeral Systems (ANS), a kind of entropy encoding algorithm, to losslessly encode the discrete latents into bitstreams for saving. 
% In this process, boring data regions will be encoded with shorter bits compare with while user interested regions will have higher bits. 


%  When scientists have memory constraints that they can not perform interactive exploration and analysis on a single workstation of the raw data, they can use Autoencoders to extract a latent representation of the raw data and perform analysis on the latent representations instead of the raw data. However, AE is a data driven method, its performance largely depends on the quality of the training data (how similar is the training data to the test data), in most cases, higher similarity indicating a high quality training data and as a result, higher quality model train on this data.  

% While any representation and tracking algorithms has errors that are inevitable, it is crucial to quantify uncertainties, and more importantly, improve the tracking quality based on estimated uncertainties. 

% Temporal prediction with reliable uncertainty estimates in the latent space. We have two assumptions: temporal smoothness and lower intrinsic dimensionality than the raw data. 
% The first assumption is based on the intuition that features move smoothly in the latent space over time. The second assumption means the features are embedded in a much lower dimensional space called latent space. With the low dimension constraint, our temporal prediction model is efficient in both computational and memory cost. 

% This paper we propose a scalable data reduction and feature tracking approach by utilizing the low dimensional latent space generated by an autoencoder. We assume that two highly related features are more likely to be close to each other in the latent space. Also, to deal with the uncertainty embedded in the representations and during the tracking process, we propose to use XX to approximation the posterior distribution of the feature over time steps. The likelihood of the candidate features are updated and the trajectories with higher likelihood is derived. 


==> tex/5_results_old.tex <==
% \begin{table*}[!ht]
% \small
% \caption{\label{tab:Datasets}Dataset name, variable name, data resolution, training epochs and time, training data size (number of blocks), encoding and decoding time on each volume (seconds). Encoding and decoding time do not induce the time used for writing/reading bitstreams files into/from disk.
%  }
% \vspace{-2pt}
% \centering
%  \begin{tabular}{c|c|c|c|c|c|c|c} 
%  Dataset & Variable & Size & Epochs & Training time & \# Training blocks & Enc. time & Dec. time \\ [0.5ex] 
%  \hline
%  Vortex & vorticity magnitude & 128$\times$128$\times$128 & 600 & 4h 20m & 1000 & 0.0232s & 0.0105s \\
%  % 3.0925s & 2.5072s
%  Nyx & log density & 256$\times$256$\times$256 & 100 & 3h 14m & 5000 & 0.2272s & 0.0794s\\
%  % 24.1848s & 20.4046s
%  Isabel & pressure & 512$\times$512$\times$96 & 200 &  5h 30m & 5500 & 0.2000s & 0.1191s\\[0.5ex]
% %  Combustion & vorticity magnitude & 480$\times$720$\times$128 & 100 & 3h 26m & 6000 & &\\
% %  Tornado & velocity & 3$\times$96$\times$96$\times$96 & 1000 & 46m 42s & 400 & & \\ [0.5ex] 
% %  \hline 
%  \end{tabular} 
%  \label{table:dataset}
% \vspace{-9pt}
% \end{table*}

\section{Results} \label{sect:Results}
% Compare the proposed method to existing super-resolution techniques and highlight its superiority in terms of visual quality and uncertainty quantification
In this section, we evaluate our proposed \sysname for particle super-resolution both quantitatively and qualitatively and compared it with several baseline methods. 


\subsection{Dataset and Training Parameters}
We evaluated our method using three scientific datasets. The datasets are listed in~\autoref{table:dataset}.

% \textbf{Vortex} is a simulation of vortex structures with spatial resolution 128$\times$128$\times$128 across 30 time steps. We used the vorticity magnitude scalar field for experiments. We randomly sampled 1000 data blocks from 5 time steps as the training data. 
\textbf{Nyx} is a cosmological simulation developed by Lawrence Berkeley National Laboratory. The log density field with a resolution 256$\times$256$\times$256 was used in our evaluation. % 5000 data blocks from 5 ensemble members were randomly sampled for training. 
% \textbf{Hurricane Isabel} is a simulation of Hurricane Isabel, produced by the Weather Research and Forecast (WRF) model, courtesy of NCAR and the U.S. National Science Foundation (NSF). The data were sliced along the z dimension to remove the special value $1 \times 10^{35}$ representing "no data" (the land region). In our experiment, the resolution of data is 512$\times$512$\times$96 with 48 time steps. We chose the pressure field for evaluation. Training data contain 5500 data blocks from 5 time steps. 
% \textbf{Turbulent Combustion} is a combustion simulation produced by Sandia National Laboratories. It is a time-varying multivariate dataset with spatial resolution 480$\times$720$\times$128 and 122 time steps. We use vorticity magnitude field for experiments, where we sample 6000 data blocks from 6 time steps for training. 

The {\sysname} model is implemented based on PyTorch$\footnote{https://pytorch.org}$ and trained on a single NVIDIA Tesla A100 GPU. The Adam optimizer~\cite{Diederik2015Adam} is used for all datasets, and the learning rate is $10^{-4}$. The total training time for each dataset is listed in~\autoref{table:dataset}.
% Based on a fully convolutional model with block-based training and inference strategy, we can apply {\sysname} on data of any resolution. 

\subsection{Quantitative Evaluation} \label{sect:QuantiEval}
In this section, we quantitatively evaluate the super-resolution result. 

\subsubsection{Evaluation Metrics}
We utilize several metrics to compare the super-resolved particles with the reference particles. We utilize standard Chamfer Distance (CD) and Earth Mover’s Distance (EMD) to measure the point-wise distances between generated high-resolution particles and the ground truth.  
CD is to measure the differences between two particle sets: for each point, the distance between it and its neighbor in another set. 
\begin{equation}
\mathrm{CD}(X,Y) = \frac{1}{|X|}\sum_{x\in X}\min_{y\in Y}||x-y||_2^2 + \frac{1}{|Y|}\sum_{y\in Y}\min_{x\in X}||x-y||_2^2
\end{equation}

EMD measures the differences between two distributions. 
\begin{equation} % TBD
\mathrm{EMD}(X, Y)=\min _{f: X \rightarrow Y} \sum _{x \in X} \left|x-f(x)\right|
\end{equation}
% where $\phi: X\to Y$ is a bijection between the two point sets that minimize the total distance between matched points, and $|\cdot|$ denotes the cardinality of a set. 
For both CD and EMD, smaller is better ($\downarrow$).

%# to be refined. 
But CD and EMD are sensitive to outliers, thus, we utilize F-score to measure the quality of super-resolution. F-score is a harmonic mean of precision and recall, where a hit (true positive) is defined by two particles existing in the  threshold radius with each other. 
\begin{equation} % TBD
\mathrm{F-score}(X, Y)=\frac{2}{\frac{1}{recall}+\frac{1}{precision}}
\end{equation}
A larger F-score is better ($\uparrow$). In our experiment, we use the radius threshold $r=0.005$.  % \delta

% 1-Nearest Neighbor Accuracy: 
We also report the Minimum Matching Distance (MMD) which is the average distance of matched particles in the ground truth and super-resolved results. 
% Coverage (COV): measures the fraction of particles in the ground truth data that is closely matched to particles in the super-resolved result.

\subsection{Baselines}
% deep learning-based approaches (GAN), nearest neighbor methods, and iterative reconstruction algorithms.

\subsection{Qualitative Evaluation}
\subsubsection{Volumetric Super-Resolution}
We qualitatively evaluate the proposed {\sysname} by volume rendering and isosurface rendering of super-resolved results. 
% with volume and isosurface rendering. 

% For all cells that are classified as filled we then distribute the total number of output samples proportionally to the density estimates of the cells. Thus our network is independent of the number of points we want to generate.

\subsection{Uncertainty Quantification}
To measure the uncertainty of {\sysname}'s super-resolution results, we utilize the standard deviation of super-resolution results from 10 runs.


\subsection{Generalization Ability}
% We evaluate the generalization ability of our method in this section. 
% The result demonstrates that the proposed model can learn particle features from XX and generalize to other unseen data in the same distribution as the training data. 
% The extracted features are robust and more efficient for downstream tasks such as particle data super-resolution and data sampling. 

% The success of our model for power-of-two SR further demonstrates the generalization of our proposed ParticleFlow. 
